Integrated Decision and Control for High-Level Automated Vehicles by Mixed Policy Gradient and Its Experiment Verification

Self-evolution is indispensable to realize full autonomous driving. This paper presents a self-evolving decision-making system based on the Integrated Decision and Control (IDC), an advanced framework built on reinforcement learning (RL). First, an RL algorithm called constrained mixed policy gradient (CMPG) is proposed to consistently upgrade the driving policy of the IDC. It adapts the MPG under the penalty method so that it can solve constrained optimization problems using both the data and model. Second, an attention-based encoding (ABE) method is designed to tackle the state representation issue. It introduces an embedding network for feature extraction and a weighting network for feature fusion, fulfilling order-insensitive encoding and importance distinguishing of road users. Finally, by fusing CMPG and ABE, we develop the first data-driven decision and control system under the IDC architecture, and deploy the system on a fully-functional self-driving vehicle running in daily operation. Experiment results show that boosting by data, the system can achieve better driving ability over model-based methods. It also demonstrates safe, efficient and smart driving behavior in various complex scenes at a signalized intersection with real mixed traffic flow.

==> data/defs.tex <==
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\lcmt}[1]{{\footnotesize\textcolor{red}{#1}}\\}
\newcommand{\todo}[1]{\cmt{(TODO: #1)}}

% 可主要定义【常用】的符号，以简化上下标、空格、左右括号等
% 以下定义的符号不用加括号，如果直接作为上下标，在正文加就好，如果不作为上下标，可能有在其上添加上下标的需求，这个时候如果加了括号，就很麻烦
\newcommand{\lb}[1]{\left [ #1 \right.}
\newcommand{\rb}[1]{\left. #1 \right ]}
\newcommand{\lrb}[1]{\left [ #1 \right ]}
\newcommand{\lp}[1]{\left ( #1 \right.}
\newcommand{\rp}[1]{\left. #1 \right )}
\newcommand{\lrp}[1]{\left ( #1 \right )}

\newcommand{\lc}[1]{\left \{ #1 \right.}
\newcommand{\rc}[1]{\left. #1 \right \}}
\newcommand{\lrc}[1]{\left \{ #1 \right \}}

\renewcommand{\lVert}[1]{\left \Vert #1 \right.}
\renewcommand{\rVert}[1]{\left. #1 \right \Vert}
\newcommand{\lrVert}[1]{\left \Vert #1 \right \Vert}

\renewcommand{\lvert}[1]{\left \vert #1 \right.}
\renewcommand{\rvert}[1]{\left. #1 \right \vert}
\newcommand{\lrvert}[1]{\left \vert #1 \right \vert}

\newcommand{\lrangle}[1]{\left \langle #1 \right \rangle}

% Math operators and functions
\newcommand{\E}[2]{\operatorname{\symbb{E}}_{#1} \lrb{#2}}
\newcommand{\D}[1]{\operatorname{\symbb{D}}\lrb{#1}}
% \newcommand{\Eleft}[2]{\operatorname{\symbb{E}}_{#1}\lb#2\right.}
% \newcommand{\Eright}[1]{\left.#1\rb}
\newcommand{\Ed}[2]{\operatorname*{\symbb{E}}_{#1} \lrb{#2}}
\newcommand{\Eleftd}[2]{\operatorname*{\symbb{E}}_{#1}\lb{#2}}
\newcommand{\Erightd}[1]{\rb{#1}}
\newcommand{\EEE}{\symbb{E}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\Max}{max}
\DeclareMathOperator*{\Min}{min}

% Other helpers
\newcommand{\voidarg}{{\,\cdot\,}}

% IDC
\newcommand{\xspace}{\symcal{X}}
\newcommand{\xspaceobst}{\symcal{X}_{\text{obst}}}
\newcommand{\x}{\symbf{x}}
\newcommand{\y}{\symbf{y}}
\newcommand{\xego}{\x_{\text{ego}}}
\newcommand{\xref}{\x_{\text{ref}}}
\newcommand{\xroad}{\x_{\text{road}}}
\newcommand{\xlight}{\x_{\text{light}}}
\newcommand{\xobst}{\x_{\text{obst}}}
\newcommand{\xobstj}{\x^j_{\text{obst}}}
\newcommand{\xobstone}{\x^1_{\text{obst}}}
\newcommand{\xobstN}{\x^N_{\text{obst}}}
\newcommand{\xobstM}{\x^M_{\text{obst}}}
\newcommand{\xset}{\x_{\text{set}}}
\newcommand{\xelse}{\x_{\text{else}}}
\newcommand{\uspace}{\symcal{U}}
\newcommand{\uaction}{\symbf{u}}
\newcommand{\uopt}{\symbf{u}\opt}
\newcommand{\ut}{\symbf{u}^t}
\newcommand{\utp}{\symbf{u}^{t+1}}
\newcommand{\tauref}{\tau_{\text{ref}}}
\newcommand{\taurefk}{\tauref^k}
\newcommand{\taurefopt}{\tau^*_{\text{ref}}}
\newcommand{\stateset}{\Pi_{\text{state}}}
\newcommand{\stateseti}{\stateset^i}
\newcommand{\statesetk}{\stateset^k}
\newcommand{\taurefset}{\Pi_{\text{ref}}}
\newcommand{\safepolicyset}{\Pi_{\text{safe}}}

\newcommand{\Jpolicy}{J_{\policy}}
\newcommand{\Jcpolicy}{J^c_{\policy}}
\newcommand{\JQ}{J_Q}
\newcommand{\pf}{\sigma}
\newcommand{\Prob}{\symcal{P}}

\newcommand{\tauhat}{\hat{\tau}}

\newcommand{\acccmd}{\Alpha}
\newcommand{\steercmd}{\Theta}



%obj：要优化的变量全在括号里面，J的上下标可以标识说明性符号，或编号，也可以不标上下标

% text
\newcommand{\obst}{\text{obst}}
\newcommand{\ego}{\text{ego}}
\newcommand{\navi}{\text{navi}}
\newcommand{\lane}{\text{lane}}
\newcommand{\rref}{\text{ref}}
\newcommand{\curve}{\text{curve}}
\renewcommand{\rule}{\text{rule}}
\newcommand{\map}{\text{map}}
\newcommand{\light}{\text{light}}
\newcommand{\road}{\text{road}}
\newcommand{\DOFWE}{\text{DOFWE}}
\newcommand{\lbd}{\text{lb}}
\newcommand{\hbd}{\text{hb}}
\newcommand{\safe}{\text{safe}}
\newcommand{\vio}{\text{vio}}
\newcommand{\pred}{\text{pred}}
\newcommand{\data}{\text{data}}
\newcommand{\model}{\text{model}}
\newcommand{\mixed}{\text{mixed}}
\newcommand{\old}{\text{old}}
\newcommand{\mpc}{\text{mpc}}
\newcommand{\track}{\text{track}}
\newcommand{\energy}{\text{energy}}
\newcommand{\stability}{\text{stability}}
\newcommand{\smooth}{\text{smooth}}
\renewcommand{\stop}{\text{stop}}

% MDP
\newcommand{\sspace}{\symcal{S}}
\newcommand{\aspace}{\symcal{A}}
\newcommand{\state}{\symbf{s}}
\newcommand{\statenoise}{\symbf{\epsilon}}
\newcommand{\sprime}{\symbf{s}^{\prime}}
\newcommand{\stm}{\state_{t-1}}
\renewcommand{\st}{\state_t}
% \renewcommand{\sl}{\state_l}
% \newcommand{\slp}{\state_{l+1}}
\newcommand{\stp}{\state_{t+1}}
\newcommand{\stpi}{\state_{t+i}}
\newcommand{\stpn}{\state_{t+n}}
\newcommand{\si}{\state_i}
\newcommand{\simm}{\state_{i-1}}
\newcommand{\sip}{\state_{i+1}}
\newcommand{\sipn}{\state_{i+n}}

\newcommand{\action}{\symbf{a}}
\newcommand{\aprime}{\symbf{a}^{\prime}}
\newcommand{\atm}{\action_{t-1}}
\newcommand{\at}{\action_t}
% \newcommand{\al}{\action_l}
\newcommand{\atp}{\action_{t+1}}
\newcommand{\atpi}{\action_{t+i}}
\newcommand{\atpn}{\action_{t+n}}
\newcommand{\ai}{\action_i}
\newcommand{\aip}{\action_{i+1}}
\newcommand{\aipn}{\action_{i+n}}
\newcommand{\opt}{^*}
\newcommand{\obs}{\symbf{o}}
\newcommand{\otm}{\obs_{t-1}}
\newcommand{\ot}{\obs_t}
% \newcommand{\ol}{\obs_l}
\newcommand{\oi}{\obs_i}
\newcommand{\oprime}{\obs^{\prime}}
\newcommand{\otp}{\obs_{t+1}}
\newcommand{\otpn}{\obs_{t+n}}

% Model correspondence for MDP
\newcommand{\statehat}{\hat{\state}}
\newcommand{\stmhat}{\statehat_{t-1}}
\newcommand{\sthat}{\statehat_t}
% \newcommand{\slhat}{\statehat_l}
\newcommand{\sihat}{\statehat_i}
\newcommand{\stphat}{\statehat_{t+1}}
\newcommand{\stpihat}{\statehat_{t+i}}
\newcommand{\slphat}{\statehat_{l+1}}
\newcommand{\siphat}{\statehat_{i+1}}
\newcommand{\stpnhat}{\statehat_{t+n}}

\newcommand{\actionhat}{\hat{\action}}
\newcommand{\atmhat}{\actionhat_{t-1}}
\newcommand{\athat}{\actionhat_t}
% \newcommand{\alhat}{\actionhat_l}
\newcommand{\aihat}{\actionhat_i}
\newcommand{\atphat}{\actionhat_{t+1}}
\newcommand{\atpihat}{\actionhat_{t+i}}
\newcommand{\atpnhat}{\actionhat_{t+n}}

% Rewards and costs
\newcommand{\reward}{r}
\newcommand{\rtm}{\reward_{t-1}}
\newcommand{\rt}{\reward_t}
% \newcommand{\rl}{\reward_l}
\newcommand{\ri}{\reward_i}
\newcommand{\rtp}{\reward_{t+1}}
\newcommand{\rtpi}{\reward_{t+i}}
\newcommand{\rtpn}{\reward_{t+n}}

\newcommand{\cost}{c}
\newcommand{\ctm}{\cost_{t-1}}
\newcommand{\ct}{\cost_t}
% \newcommand{\cl}{\cost_l}
\newcommand{\ci}{\cost_i}
\newcommand{\ctp}{\cost_{t+1}}
\newcommand{\ctpi}{\cost_{t+i}}
\newcommand{\ctpn}{\cost_{t+n}}

% Model correspondence for Rewards and costs
\newcommand{\rewardhat}{\hat{r}}
\newcommand{\rtmhat}{\rewardhat_{t-1}} 
\newcommand{\rthat}{\rewardhat_t}
% \newcommand{\rlhat}{\rewardhat_l}
\newcommand{\rihat}{\rewardhat_i}
\newcommand{\rtphat}{\rewardhat_{t+1}}
\newcommand{\rtpihat}{\rewardhat_{t+i}}
\newcommand{\rtpnhat}{\rewardhat_{t+n}}

\newcommand{\costhat}{\hat{c}}
\newcommand{\ctmhat}{\costhat_{t-1}}
\newcommand{\cthat}{\costhat_t}
\newcommand{\clhat}{\costhat_l}
\newcommand{\cihat}{\costhat_i}
\newcommand{\ctphat}{\costhat_{t+1}}
\newcommand{\ctpihat}{\costhat_{t+i}}
\newcommand{\ctpnhat}{\costhat_{t+n}}

% V function
\newcommand{\vpolicy}{v^{\policy}}
\newcommand{\vpolicywithparams}{v^{\policywithparams}}
\newcommand{\Vwithparams}{V_{\vparams}}

\newcommand{\vdiamond}{v_{\diamond}}
\newcommand{\vdiamondopt}{\vdiamond\opt}
\newcommand{\vdiamondpolicy}{\vdiamond^{\policy}}
\newcommand{\vdiamondpolicywithparams}{\vdiamond^{\policywithparams}}
\newcommand{\Vdiamond}{V_{\diamond}}
\newcommand{\Vwithdiamondparams}{V_{\vdiamondparams}}

\newcommand{\vr}{v_r}
\newcommand{\vropt}{\vr\opt}
\newcommand{\vrpolicy}{\vr^{\policy}}
\newcommand{\vrpolicywithparams}{\vr^{\policywithparams}}
\newcommand{\Vr}{V_r}
\newcommand{\Vwithrparams}{V_{\vrparams}}

\newcommand{\vc}{v_c}
\newcommand{\vcopt}{\vc\opt}
\newcommand{\vcpolicy}{\vc^{\policy}}
\newcommand{\vcpolicywithparams}{\vc^{\policywithparams}}
\newcommand{\Vc}{V_c}
\newcommand{\Vwithcparams}{V_{\vcparams}}

% Q function
\newcommand{\qpolicy}{q^{\policy}}
\newcommand{\qpolicywithparams}{q^{\policywithparams}}
\newcommand{\Qwithparams}{Q_{\qparams}}

\newcommand{\qdiamond}{q_{\diamond}}
\newcommand{\qdiamondopt}{\qdiamond^*}
\newcommand{\qdiamondpolicy}{q^{\policy}_{\diamond}}
\newcommand{\Qdiamond}{Q_{\diamond}}
\newcommand{\Qwithdiamondparams}{Q_{\qdiamondparams}}

\newcommand{\qr}{q_r}
\newcommand{\qropt}{\qr^*}
\newcommand{\qrpolicy}{q^{\policy}_r}
\newcommand{\qrpolicywithparams}{q^{\policywithparams}_r}

\newcommand{\Qr}{Q_r}
\newcommand{\Qwithrparams}{Q_{\qrparams}}
\newcommand{\Qwithrparamsopt}{Q_{\qrparamsopt}}

\newcommand{\qc}{q_c}
\newcommand{\qcopt}{\qc\opt}
\newcommand{\qcpolicy}{q^{\policy}_c}
\newcommand{\qcpolicywithparams}{q^{\policywithparams}_c}
\newcommand{\Qc}{Q_c}
\newcommand{\Qwithcparams}{Q_{\qcparams}}
\newcommand{\Qwithcparamsopt}{Q_{\qcparamsopt}}

% Policy and params
\newcommand{\policy}{\pi}
\newcommand{\policyopt}{\policy^*}
\newcommand{\policycirc}{\policy^{\circ}}
\newcommand{\policywithparams}{\policy_{\pparams}}
\newcommand{\policywithparamsopt}{\policy_{\pparamsopt}}
\newcommand{\pparams}{\symbf{\theta}}
\newcommand{\pparamsopt}{\pparams\opt}

\newcommand{\qparams}{\symbf{\omega}}
\newcommand{\qparamsopt}{\qparams\opt}
\newcommand{\qdiamondparams}{\qparams_{\diamond}}
\newcommand{\qrparams}{\qparams_r}
\newcommand{\qcparams}{\qparams_c}
\newcommand{\qrparamsopt}{\qparams\opt_r}
\newcommand{\qcparamsopt}{\qparams\opt_c}
\newcommand{\qrparamspolicywithparams}{\qparams_r^{\policywithparams}}
\newcommand{\qcparamspolicywithparams}{\qparams_c^{\policywithparams}}


% \newcommand{\qoneparams}{{\omega^1}}
% \newcommand{\qtwoparams}{{\omega^1}}
% \newcommand{\qonerparams}{{\omega^1_r}}
% \newcommand{\qtworparams}{{\omega^2_r}}
% \newcommand{\qonecparams}{{\omega^1_c}}
% \newcommand{\qtwocparams}{{\omega^2_c}}

\newcommand{\vparams}{\symbf{\omega}}
\newcommand{\vdiamondparams}{\vparams_{\diamond}}
\newcommand{\vrparams}{\vparams_r}
\newcommand{\vcparams}{\vparams_c}

\newcommand{\ptargetparams}{\bar{\pparams}}

\newcommand{\qtargetparams}{\bar{\qparams}}
\newcommand{\qrtargetparams}{\bar{\qrparams}}
\newcommand{\qctargetparams}{\bar{\qcparams}}

% \newcommand{\qonetargetparams}{{\bar\qoneparams}}
% \newcommand{\qtwotargetparams}{{\bar\qtwoparams}}
% \newcommand{\qonertargetparams}{{\bar\qonerparams}}
% \newcommand{\qtwortargetparams}{{\bar\qtworparams}}
% \newcommand{\qonectargetparams}{{\bar\qonecparams}}
% \newcommand{\qtwoctargetparams}{{\bar\qtwocparams}}

\newcommand{\vtargetparams}{\bar{\vparams}}
\newcommand{\vrtargetparams}{\bar{\vrparams}}
\newcommand{\vctargetparams}{\bar{\vcparams}}

\newcommand{\Qhatwtpn}{\hat{Q}_{\qparams,t+n}}
\newcommand{\Qhatwtp}{\hat{Q}_{\qparams,t+1}}
\newcommand{\Qhatwt}{\hat{Q}_{\qparams,t}}
\newcommand{\Qhatwtpi}{\hat{Q}_{\qparams,t+i}}

% encoding params
\newcommand{\eparams}{\symbf{\psi}}


% Distributions.
\newcommand{\gauss}{\symcal{N}}
\newcommand{\buffer}{\symcal{B}}
\newcommand{\ifelse}{\symbb{I}}
\newcommand{\targetnetsyncrate}{\iota}


% Other.
\newcommand{\inv}{^{-1}}
\newcommand{\T}{^{\top}}
\newcommand{\reals}{\symbb{R}}
\newcommand{\discount}{\gamma}
\newcommand{\Exp}{\mathop{\mathbb E}\displaylimits}
\newcommand{\dvf}{\rho^{\policy}(\state)}
\newcommand{\dvfwithparams}{\rho^{\policywithparams}(\state)}

\newcommand{\VNE}{\text{V}_{\text{NE}}}
\newcommand{\VNS}{\text{V}_{\text{NS}}}
\newcommand{\VNW}{\text{V}_{\text{NW}}}
\newcommand{\VES}{\text{V}_{\text{ES}}}
\newcommand{\VEW}{\text{V}_{\text{EW}}}
\newcommand{\VEN}{\text{V}_{\text{EN}}}
\newcommand{\VSW}{\text{V}_{\text{SW}}}
\newcommand{\VSN}{\text{V}_{\text{SN}}}
\newcommand{\VSE}{\text{V}_{\text{SE}}}
\newcommand{\VWN}{\text{V}_{\text{WN}}}
\newcommand{\VWE}{\text{V}_{\text{WE}}}
\newcommand{\VWS}{\text{V}_{\text{WS}}}

\newcommand{\BNS}{\text{B}_{\text{NS}}}
\newcommand{\BEW}{\text{B}_{\text{EW}}}
\newcommand{\BSN}{\text{B}_{\text{SN}}}
\newcommand{\BWE}{\text{B}_{\text{WE}}}

\newcommand{\PNW}{\text{P}_{\text{NW}}}
\newcommand{\PNE}{\text{P}_{\text{NE}}}
\newcommand{\PEN}{\text{P}_{\text{EN}}}
\newcommand{\PES}{\text{P}_{\text{ES}}}
\newcommand{\PSE}{\text{P}_{\text{SE}}}
\newcommand{\PSW}{\text{P}_{\text{SW}}}
\newcommand{\PWS}{\text{P}_{\text{WS}}}
\newcommand{\PWN}{\text{P}_{\text{WN}}}

